Timelike singularities and Hamiltonian cosmological billiards

We construct a large class of vacuum solutions of the Einstein equations without any symmetries and with controlled asymptotics near a timelike singularity. The solutions are obtained by a Fuchs analysis of the equations which evolve the metric in a spacelike direction. We further observe that the changes of signs of some of the terms (walls) in the associated Hamiltonian invalidate the "cosmological billards" heuristic arguments for existence of singularities of mixmaster type in the current context.

==> neounicodedefs.tex <==
\usepackage{newunicodechar}
\newunicodechar{∂}{\partial}
\newunicodechar{∀}{\forall}
\newunicodechar{×}{\times}
\newunicodechar{α}{\alpha}
\newunicodechar{β}{\beta}
\newunicodechar{γ}{\gamma}
\newunicodechar{δ}{\delta}
\newunicodechar{ε}{\epsilon}
\newunicodechar{η}{\eta}
\newunicodechar{φ}{\varphi}
\newunicodechar{ϕ}{\phi}
\newunicodechar{λ}{\lambda}
\newunicodechar{ψ}{\psi}
\newunicodechar{ρ}{\rho}
\newunicodechar{ω}{\omega}
\newunicodechar{τ}{\tau}
\newunicodechar{θ}{\theta}
\newunicodechar{μ}{\mu}
\newunicodechar{ν}{\nu}
\newunicodechar{π}{\pi}
\newunicodechar{σ}{\sigma}
\newunicodechar{ξ}{\xi}
\newunicodechar{Γ}{\Gamma}
\newunicodechar{Ψ}{\Psi}
\newunicodechar{Ω}{\Omega}
\newunicodechar{Σ}{\Sigma}
\newunicodechar{Θ}{\Theta}
\newunicodechar{Λ}{\Lambda}
